Focusing Knowledge-based Graph Argument Mining via Topic Modeling

Decision-making usually takes five steps: identifying the problem, collecting data, extracting evidence, identifying pro and con arguments, and making decisions. Focusing on extracting evidence, this paper presents a hybrid model that combines latent Dirichlet allocation and word embeddings to obtain external knowledge from structured and unstructured data. We study the task of sentence-level argument mining, as arguments mostly require some degree of world knowledge to be identified and understood. Given a topic and a sentence, the goal is to classify whether a sentence represents an argument in regard to the topic. We use a topic model to extract topic- and sentence-specific evidence from the structured knowledge base Wikidata, building a graph based on the cosine similarity between the entity word vectors of Wikidata and the vector of the given sentence. Also, we build a second graph based on topic-specific articles found via Google to tackle the general incompleteness of structured knowledge bases. Combining these graphs, we obtain a graph-based model which, as our evaluation shows, successfully capitalizes on both structured and unstructured data.

==> results.tex <==
============= PATHS ==============
{'wd': {'Ns_s': 0.14375,
        'Ns_t': 0.8612500000000001,
        'hops': 7.286268844221105,
        'len': 1.6169166183481511,
        's_s': 0.33125,
        's_t': 0.38125,
        'time': 30.162553391959797},
 'wd_lda': {'Ns_s': 1.145,
            'Ns_t': 1.3875,
            'hops': 5.145542353263781,
            'len': 3.7654758203589833,
            's_s': 0.44,
            's_t': 0.5125,
            'time': 276.2127045442951},
 'wd_lda_glove': {'Ns_s': 1.4662816499057267,
                  'Ns_t': 1.5705247179827992,
                  'hops': 6.444687349868836,
                  'len': 4.4515008680564145,
                  's_s': 0.48875,
                  's_t': 0.5462499999999999,
                  'time': 301.75220078207667},
 'wd_lda_glove_openie': {'Ns_s': 6.889318467336684,
                         'Ns_t': 9.791639447236182,
                         'hops': 6.661623743718593,
                         'len': 7.169459055080519,
                         's_s': 0.80375,
                         's_t': 0.7012499999999999,
                         'time': 334.5219252512563}}
============== AVG ===============
{'wd': {'acc': 0.7808,
               'f1_macro_dev': 0.7074,
               'f1_macro_test': 0.6341,
               'loss': 0.4809,
               'val_acc': 0.7103,
               'val_loss': 0.5958},
 'wd_lda': {'acc': 0.7955,
               'f1_macro_dev': 0.6797,
               'f1_macro_test': 0.6571,
               'loss': 0.4426,
               'val_acc': 0.6854,
               'val_loss': 0.6429},
 'wd_lda_glove': {'acc': 0.8172,
               'f1_macro_dev': 0.6796,
               'f1_macro_test': 0.63,
               'loss': 0.4173,
               'val_acc': 0.6984,
               'val_loss': 0.6563},
 'wd_lda_glove_openie': {'acc': 0.8504,
               'f1_macro_dev': 0.6767,
               'f1_macro_test': 0.6785,
               'loss': 0.3537,
               'val_acc': 0.6802,
               'val_loss': 0.693}}
============== STDS ==============
{'wd': {'acc': 0.0087,
               'f1_macro_dev': 0.0071,
               'f1_macro_test': 0.0096,
               'loss': 0.0136,
               'val_acc': 0.0082,
               'val_loss': 0.0243},
 'wd_lda': {'acc': 0.0066,
               'f1_macro_dev': 0.0079,
               'f1_macro_test': 0.0184,
               'loss': 0.009,
               'val_acc': 0.0131,
               'val_loss': 0.025},
 'wd_lda_glove': {'acc': 0.0145,
               'f1_macro_dev': 0.0173,
               'f1_macro_test': 0.033,
               'loss': 0.0214,
               'val_acc': 0.011,
               'val_loss': 0.0304},
 'wd_lda_glove_openie': {'acc': 0.0104,
               'f1_macro_dev': 0.012,
               'f1_macro_test': 0.0214,
               'loss': 0.0125,
               'val_acc': 0.0112,
               'val_loss': 0.0212}}
============== STATS =============
{'wd': {'abortion': {'acc': 0.7534,
                            'f1_macro_dev': 0.7141,
                            'f1_macro_test': 0.6454,
                            'loss': 0.5163,
                            'val_acc': 0.7187,
                            'val_loss': 0.5541},
               'cloning': {'acc': 0.7742,
                           'f1_macro_dev': 0.6749,
                           'f1_macro_test': 0.6424,
                           'loss': 0.4895,
                           'val_acc': 0.7024,
                           'val_loss': 0.5862},
               'death_penalty': {'acc': 0.8162,
                                 'f1_macro_dev': 0.7103,
                                 'f1_macro_test': 0.6191,
                                 'loss': 0.4187,
                                 'val_acc': 0.6965,
                                 'val_loss': 0.6128},
               'gun_control': {'acc': 0.7904,
                               'f1_macro_dev': 0.7104,
                               'f1_macro_test': 0.7502,
                               'loss': 0.4746,
                               'val_acc': 0.7059,
                               'val_loss': 0.6},
               'marijuana_legalization': {'acc': 0.7927,
                                          'f1_macro_dev': 0.7077,
                                          'f1_macro_test': 0.6837,
                                          'loss': 0.4659,
                                          'val_acc': 0.7177,
                                          'val_loss': 0.5915},
               'minimum_wage': {'acc': 0.7751,
                                'f1_macro_dev': 0.6914,
                                'f1_macro_test': 0.5534,
                                'loss': 0.4921,
                                'val_acc': 0.6865,
                                'val_loss': 0.6436},
               'nuclear_energy': {'acc': 0.7506,
                                  'f1_macro_dev': 0.7136,
                                  'f1_macro_test': 0.7186,
                                  'loss': 0.5237,
                                  'val_acc': 0.7162,
                                  'val_loss': 0.6237},
               'school_uniforms': {'acc': 0.7939,
                                   'f1_macro_dev': 0.737,
                                   'f1_macro_test': 0.4604,
                                   'loss': 0.4668,
                                   'val_acc': 0.7387,
                                   'val_loss': 0.5544}},
 'wd_lda': {'abortion': {'acc': 0.7993,
                            'f1_macro_dev': 0.6832,
                            'f1_macro_test': 0.6787,
                            'loss': 0.4322,
                            'val_acc': 0.6826,
                            'val_loss': 0.6221},
               'cloning': {'acc': 0.7917,
                           'f1_macro_dev': 0.6877,
                           'f1_macro_test': 0.6503,
                           'loss': 0.4455,
                           'val_acc': 0.6709,
                           'val_loss': 0.6593},
               'death_penalty': {'acc': 0.7937,
                                 'f1_macro_dev': 0.7024,
                                 'f1_macro_test': 0.6315,
                                 'loss': 0.4561,
                                 'val_acc': 0.7055,
                                 'val_loss': 0.5877},
               'gun_control': {'acc': 0.7939,
                               'f1_macro_dev': 0.6657,
                               'f1_macro_test': 0.6655,
                               'loss': 0.4557,
                               'val_acc': 0.6941,
                               'val_loss': 0.6091},
               'marijuana_legalization': {'acc': 0.8114,
                                          'f1_macro_dev': 0.6859,
                                          'f1_macro_test': 0.7537,
                                          'loss': 0.4289,
                                          'val_acc': 0.6929,
                                          'val_loss': 0.6622},
               'minimum_wage': {'acc': 0.7826,
                                'f1_macro_dev': 0.6364,
                                'f1_macro_test': 0.7488,
                                'loss': 0.4556,
                                'val_acc': 0.6785,
                                'val_loss': 0.6657},
               'nuclear_energy': {'acc': 0.7937,
                                  'f1_macro_dev': 0.6917,
                                  'f1_macro_test': 0.6149,
                                  'loss': 0.4295,
                                  'val_acc': 0.6725,
                                  'val_loss': 0.7012},
               'school_uniforms': {'acc': 0.7979,
                                   'f1_macro_dev': 0.6849,
                                   'f1_macro_test': 0.5136,
                                   'loss': 0.437,
                                   'val_acc': 0.6863,
                                   'val_loss': 0.6359}},
 'wd_lda_glove': {'abortion': {'acc': 0.8131,
                            'f1_macro_dev': 0.6975,
                            'f1_macro_test': 0.7295,
                            'loss': 0.4323,
                            'val_acc': 0.7006,
                            'val_loss': 0.6317},
               'cloning': {'acc': 0.818,
                           'f1_macro_dev': 0.6799,
                           'f1_macro_test': 0.643,
                           'loss': 0.4217,
                           'val_acc': 0.6965,
                           'val_loss': 0.6413},
               'death_penalty': {'acc': 0.8207,
                                 'f1_macro_dev': 0.712,
                                 'f1_macro_test': 0.5904,
                                 'loss': 0.4103,
                                 'val_acc': 0.7066,
                                 'val_loss': 0.6621},
               'gun_control': {'acc': 0.815,
                               'f1_macro_dev': 0.6182,
                               'f1_macro_test': 0.6031,
                               'loss': 0.4269,
                               'val_acc': 0.6802,
                               'val_loss': 0.667},
               'marijuana_legalization': {'acc': 0.8177,
                                          'f1_macro_dev': 0.6792,
                                          'f1_macro_test': 0.6581,
                                          'loss': 0.4254,
                                          'val_acc': 0.6876,
                                          'val_loss': 0.6883},
               'minimum_wage': {'acc': 0.7899,
                                'f1_macro_dev': 0.6822,
                                'f1_macro_test': 0.7362,
                                'loss': 0.4283,
                                'val_acc': 0.7005,
                                'val_loss': 0.6449},
               'nuclear_energy': {'acc': 0.8272,
                                  'f1_macro_dev': 0.6805,
                                  'f1_macro_test': 0.5951,
                                  'loss': 0.4113,
                                  'val_acc': 0.6949,
                                  'val_loss': 0.652},
               'school_uniforms': {'acc': 0.836,
                                   'f1_macro_dev': 0.6871,
                                   'f1_macro_test': 0.4845,
                                   'loss': 0.3822,
                                   'val_acc': 0.7203,
                                   'val_loss': 0.6635}},
 'wd_lda_glove_openie': {'abortion': {'acc': 0.8726,
                            'f1_macro_dev': 0.6486,
                            'f1_macro_test': 0.6916,
                            'loss': 0.3205,
                            'val_acc': 0.655,
                            'val_loss': 0.7143},
               'cloning': {'acc': 0.85,
                           'f1_macro_dev': 0.6724,
                           'f1_macro_test': 0.7224,
                           'loss': 0.3691,
                           'val_acc': 0.6753,
                           'val_loss': 0.6923},
               'death_penalty': {'acc': 0.863,
                                 'f1_macro_dev': 0.6867,
                                 'f1_macro_test': 0.6415,
                                 'loss': 0.3354,
                                 'val_acc': 0.7146,
                                 'val_loss': 0.6583},
               'gun_control': {'acc': 0.8542,
                               'f1_macro_dev': 0.696,
                               'f1_macro_test': 0.7476,
                               'loss': 0.3355,
                               'val_acc': 0.6752,
                               'val_loss': 0.7427},
               'marijuana_legalization': {'acc': 0.8225,
                                          'f1_macro_dev': 0.6421,
                                          'f1_macro_test': 0.63,
                                          'loss': 0.423,
                                          'val_acc': 0.6558,
                                          'val_loss': 0.6921},
               'minimum_wage': {'acc': 0.815,
                                'f1_macro_dev': 0.6705,
                                'f1_macro_test': 0.7712,
                                'loss': 0.4013,
                                'val_acc': 0.667,
                                'val_loss': 0.6625},
               'nuclear_energy': {'acc': 0.85,
                                  'f1_macro_dev': 0.6955,
                                  'f1_macro_test': 0.7045,
                                  'loss': 0.3402,
                                  'val_acc': 0.6965,
                                  'val_loss': 0.6794},
               'school_uniforms': {'acc': 0.876,
                                   'f1_macro_dev': 0.7022,
                                   'f1_macro_test': 0.5194,
                                   'loss': 0.3042,
                                   'val_acc': 0.7024,
                                   'val_loss': 0.7026}}}
